START: Self-taught Reasoner with Tools

Large reasoning models (LRMs) like OpenAI-o1 and DeepSeek-R1 have demonstrated remarkable capabilities in complex reasoning tasks through the utilization of long Chain-of-thought (CoT). However, these models often suffer from hallucinations and inefficiencies due to their reliance solely on internal reasoning processes. In this paper, we introduce START (Self-Taught Reasoner with Tools), a novel tool-integrated long CoT reasoning LLM that significantly enhances reasoning capabilities by leveraging external tools. Through code execution, START is capable of performing complex computations, self-checking, exploring diverse methods, and self-debugging, thereby addressing the limitations of LRMs. The core innovation of START lies in its self-learning framework, which comprises two key techniques: 1) Hint-infer: We demonstrate that inserting artificially designed hints (e.g., ``Wait, maybe using Python here is a good idea.'') during the inference process of a LRM effectively stimulates its ability to utilize external tools without the need for any demonstration data. Hint-infer can also serve as a simple and effective sequential test-time scaling method; 2) Hint Rejection Sampling Fine-Tuning (Hint-RFT): Hint-RFT combines Hint-infer and RFT by scoring, filtering, and modifying the reasoning trajectories with tool invocation generated by a LRM via Hint-infer, followed by fine-tuning the LRM. Through this framework, we have fine-tuned the QwQ-32B model to achieve START. On PhD-level science QA (GPQA), competition-level math benchmarks (AMC23, AIME24, AIME25), and the competition-level code benchmark (LiveCodeBench), START achieves accuracy rates of 63.6%, 95.0%, 66.7%, 47.1%, and 47.3%, respectively. It significantly outperforms the base QwQ-32B and achieves performance comparable to the state-of-the-art open-weight model R1-Distill-Qwen-32B and the proprietary model o1-Preview.

==> basemodel.tex <==
\begin{table*}[!t]
\centering
\caption{Compare different base model on challenging reasoning tasks, including PhD-level science QA, math, and code benchmarks. We report Pass@1 metric for all tasks.}
\label{tab:differntbase}
\setlength\tabcolsep{1.7pt}
\fontsize{8.1pt}{10.5pt}\selectfont
\begin{tabular}{p{2.65cm}cccccccccccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{GPQA (PhD-Level Science QA)}} & \multicolumn{3}{c}{\textbf{Math Benchmarks}} & \multicolumn{4}{c}{\textbf{LiveCodeBench}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-12}
 & Physics & Chemistry & Biology & Overall & MATH500 & AMC23 & AIME24 & Easy & Medium & Hard & Overall \\
\midrule
QwQ-32B-Preview & 75.6 & 39.8 & 68.4 & 58.1 & 90.6 & 82.5 & 50.0 & \underline{-} & \underline{-} & \textbf{-} & 41.4 \\
\midrule
START-from-base & - & - & - & - & - & - & - & \underline{-} & \underline{-} & \textbf{-} & - \\
\midrule
START-from-r1 & - & - & - & - & - & - & - & \underline{-} & \underline{-} & \textbf{-} & - \\
\midrule
START (Ours) & \textbf{80.0} & \textbf{46.2} & \textbf{68.4} & \textbf{63.6} & \textbf{94.4} & \textbf{95.0} & \textbf{66.7} &  & \textbf{} & \textbf{} & \textbf{46.4} \\
% \rowcolor[RGB]{236,244,252} 
% Search-o1-Light & \multicolumn{11}{l}{\textit{Results Coming Soon}} \\
\bottomrule
\end{tabular}
\end{table*}

==> hint-lib.tex <==
% \documentclass{article}
% \usepackage{longtable}
% \usepackage{geometry}
% \usepackage{array}
% \usepackage{booktabs}
% \usepackage{ragged2e}

% \geometry{a4paper, margin=1in}

% % \begin{document}

\begin{longtable}{ p{0.7\textwidth} p{0.25\textwidth} }
\caption{Hint-Library} \\
\toprule
\textbf{Hint} & \textbf{Label} \\
\midrule
\endfirsthead

\multicolumn{2}{c}%
{{\bfseries Table \thetable\ Continued from previous page}} \\
\toprule
\textbf{Hint} & \textbf{Label} \\
\midrule
\endhead

\midrule \multicolumn{2}{r}{{Continued on next page}} \\
\endfoot

\bottomrule
\endlastfoot

\texttt{\textbackslash nLet me first write a code that includes all test cases from the problems to validate my reasoning locally.\textbackslash nTo ensure that my code runs correctly, I need to embed all test case inputs directly into my code and print the corresponding output, following the sample structure below:\textbackslash n\textbackslash n\texttt{```python}\\
def function\_name(parameters):\\
\quad \# Implementation\\
\quad return result\\
\textbackslash n\textbackslash n\# Example input\\
test\_input1 = [\ldots] \\
\# Print output\\
\textbackslash n\textbackslash nprint(function\_name(test\_input1)) \\
test\_input2 = [\ldots] \\
\# Print output\\
\textbackslash n\textbackslash nprint(function\_name(test\_input2)) \# Check the output\\
\texttt{```}\\
\texttt{```output}\\
[\ldots]\\
\texttt{```}\\
Alright, with this structure, I can write and execute my code in a Python compiler using real example inputs. By comparing the actual outputs with the expected outputs, I can initially assess the correctness of my code. If the outputs do not match, I can debug accordingly. Recall the test cases in the problem statement.\{testcase\}. Alright, now I can write a debug code with samples input.\\
\texttt{```python} & Code: Debug Hint (Without Starter Code) \\

\texttt{\textbackslash nLet me first write a code that includes all test cases from the problems to validate my reasoning locally.\textbackslash nTo ensure that my code runs correctly, I need to embed all test case inputs directly into my code and print the corresponding output, following the sample structure below:\textbackslash n\textbackslash n\{startcoder\}\\
\# Test the example inputs\\
solution = Solution()\\
\# Example input1\\
test\_input1 = \ldots\\
\# Print output\\
\textbackslash n\textbackslash nprint(solution.function\_name(test\_input1))\\
test\_input2 = \ldots\\
\# Print output\\
\textbackslash n\textbackslash nprint(solution.function\_name(test\_input2)) \# Check the output\\
\texttt{```}\\
\texttt{```output}\\
[\ldots]\\
\texttt{```}\\
Alright, with this structure, I can write and execute my code in a Python compiler using real example inputs. By comparing the actual outputs with the expected outputs, I can initially assess the correctness of my code. If the outputs do not match, I can debug accordingly. Recall the test cases in the problem statement.\{testcase\}. Alright, now I can write a debug code with samples input.\\
\texttt{```python} & Code: Debug Hint (With Starter Code) \\

, I can use Python to perform complex calculations for this problem.\textbackslash n\texttt{```python} & Math: Complex Calculations Prompt 1 \\

, let me utilize Python to handle the intricate computations required here.\textbackslash n\texttt{```python} & Math: Complex Calculations Prompt 2 \\

, using Python, I can compute the necessary advanced mathematical operations.\textbackslash n\texttt{```python} & Math: Complex Calculations Prompt 3 \\

, maybe Python can assist in executing the detailed calculations needed.\textbackslash n\texttt{```python} & Math: Complex Calculations Prompt 4 \\

, I can employ Python to carry out the extensive numerical computations.\textbackslash n\texttt{```python} & Math: Complex Calculations Prompt 5 \\

, let me utilize Python to reflect on our current approach and identify potential improvements.\textbackslash n\texttt{```python} & Math: Reflection Prompt 1 \\

, using Python, I can analyze our strategy to find areas for enhancement.\textbackslash n\texttt{```python} & Math: Reflection Prompt 2 \\

, maybe Python can help in evaluating the effectiveness of our current method.\textbackslash n\texttt{```python} & Math: Reflection Prompt 3 \\

, I can use Python to assess and refine our problem-solving approach.\textbackslash n\texttt{```python} & Math: Reflection Prompt 4 \\

, let me employ Python to introspect our reasoning process for better insights.\textbackslash n\texttt{```python} & Math: Reflection Prompt 5 \\

, using Python, I can verify the logical consistency of our previous steps.\textbackslash n\texttt{```python} & Math: Check Previous Logic Prompt 1 \\

, let me employ Python to check the logic we've applied so far.\textbackslash n\texttt{```python} & Math: Check Previous Logic Prompt 2 \\

, maybe Python can assist in ensuring our logical deductions are sound.\textbackslash n\texttt{```python} & Math: Check Previous Logic Prompt 3 \\

, I can use Python to validate the logical flow of our solution.\textbackslash n\texttt{```python} & Math: Check Previous Logic Prompt 4 \\

, let me utilize Python to review the coherence of our reasoning.\textbackslash n\texttt{```python} & Math: Check Previous Logic Prompt 5 \\

, I can use Python to explore an alternative method for solving this problem.\textbackslash n\texttt{```python} & Math: Alternative Method Prompt 1 \\

, using Python, I can experiment with a different approach to tackle this challenge.\textbackslash n\texttt{```python} & Math: Alternative Method Prompt 2 \\

, maybe Python can assist in adopting a new strategy to find the solution.\textbackslash n\texttt{```python} & Math: Alternative Method Prompt 3 \\

, let me utilize Python to implement another method for addressing this issue.\textbackslash n\texttt{```python} & Math: Alternative Method Prompt 4 \\

, I can employ Python to try a different technique for solving this equation.\textbackslash n\texttt{```python} & Math: Alternative Method Prompt 5 \\

, Let me utilize Python to try a different approach to this step.\textbackslash n\texttt{```python} & Math: Alternative Method Prompt 6 \\

, using Python, I can experiment with a new method to tackle this challenge.\textbackslash n\texttt{```python} & Math: Alternative Method Prompt 7 \\

, maybe Python can assist in finding a different pathway to the solution.\textbackslash n\texttt{```python} & Math: Alternative Method Prompt 8 \\

Wait, I can think more deeply about this problem through python tools.\textbackslash n\texttt{```python} & Math: Deeper Think Hint 1 \\

Wait, let me think more deeply and recheck my solution through python tools.\textbackslash n\texttt{```python} & Math: Deeper Think Hint 2 \\

maybe using python here is a good idea.\textbackslash n\texttt{```python} & Math: General Hint \\

\end{longtable}

% \end{document}


==> tab_main_results.tex <==
\begin{table*}[!t]
\centering
\caption{Main results on challenging reasoning tasks, including PhD-level science QA, math, and code benchmarks. We report Pass@1 metric for all tasks. For models with 32B parameters, the best results are in \textbf{bold} and the second-best are \underline{underlined}. Results from larger or non-proprietary models are in \textcolor{gray!135}{gray} color for reference. Symbol ``$^\dagger$'' indicates results from their official releases.}
\label{tab:reasoning_performance}
\setlength\tabcolsep{1.7pt}
\fontsize{8.1pt}{10.5pt}\selectfont
\begin{tabular}{p{2.65cm}cccccccccccc}
\toprule
\multirow{2}[2]{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{GPQA (PhD-Level Science QA)}} & \multicolumn{3}{c}{\textbf{Math Benchmarks}} & \multicolumn{4}{c}{\textbf{LiveCodeBench}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-12}
 & Physics & Chemistry & Biology & Overall & MATH500 & AMC23 & AIME24 & Easy & Medium & Hard & Overall \\
\midrule
\multicolumn{12}{c}{\textit{\textbf{General LLMs}}} \\
\midrule
Qwen2.5-32B & 57.0 & 33.3 & 52.6 & 46.4 & 75.8 & 57.5 & 23.3 & 42.3 & 18.9 & \underline{14.3} & 22.3 \\
Qwen2.5-Coder-32B & 37.2 & 25.8 & 57.9 & 33.8 & 71.2 & 67.5 & 20.0 & \underline{61.5} & 16.2 & 12.2 & 25.0 \\
Qwen2.5-MATH-72B & - & - & - & - & 88.1 & - & - & \underline{-} & - & - & - \\
Qwen2.5-72B & \textcolor{gray!135}{57.0} & \textcolor{gray!135}{37.6} & \textcolor{gray!135}{68.4} & \textcolor{gray!135}{49.0} & \textcolor{gray!135}{79.4} & \textcolor{gray!135}{67.5} & \textcolor{gray!135}{20.0} & \textcolor{gray!135}{53.8} & \textcolor{gray!135}{29.7} & \textcolor{gray!135}{24.5} & \textcolor{gray!135}{33.0} \\
Llama3.3-70B & \textcolor{gray!135}{54.7} & \textcolor{gray!135}{31.2} & \textcolor{gray!135}{52.6} & \textcolor{gray!135}{43.4} & \textcolor{gray!135}{70.8} & \textcolor{gray!135}{47.5} & \textcolor{gray!135}{36.7} & \textcolor{gray!135}{57.7} & \textcolor{gray!135}{32.4} & \textcolor{gray!135}{24.5} & \textcolor{gray!135}{34.8} \\
% DeepSeek-V3-671B & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{59.1} & \textcolor{gray!135}{90.2} & \textcolor{gray!135}{-} & \textcolor{gray!135}{39.2} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{40.5} \\
DeepSeek-V3-671B & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{59.1} & \textcolor{gray!135}{90.2} & \textcolor{gray!135}{-} & \textcolor{gray!135}{39.2} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{40.5} \\
GPT-4o$^\dagger$ & \textcolor{gray!135}{59.5} & \textcolor{gray!135}{40.2} & \textcolor{gray!135}{61.6} & \textcolor{gray!135}{50.6} & \textcolor{gray!135}{60.3} & \textcolor{gray!135}{-} & \textcolor{gray!135}{9.3} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{33.4} \\
\midrule
\multicolumn{12}{c}{\textit{\textbf{Reasoning LLMs}}} \\
% \midrule
\midrule
\multicolumn{12}{l}{\textit{API Only}} \\
\midrule
o1-preview$^\dagger$ & \textcolor{gray!135}{89.4} & \textcolor{gray!135}{59.9} & \textcolor{gray!135}{65.9} & \textcolor{gray!135}{73.3} & \textcolor{gray!135}{85.5} & \textcolor{gray!135}{-} & \textcolor{gray!135}{44.6} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{53.6} \\
o1-mini$^\dagger$ & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{90.0} & \textcolor{gray!135}{-} & \textcolor{gray!135}{63.6} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} \\
o3-mini(low)$^\dagger$ & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{70.6} & \textcolor{gray!135}{95.8} & \textcolor{gray!135}{-} & \textcolor{gray!135}{60.0} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{75.6} \\
DeepSeek-R1-Lite$^\dagger$ & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{58.5} & \textcolor{gray!135}{91.6} & \textcolor{gray!135}{-} & \textcolor{gray!135}{52.5} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{51.6} \\
% \midrule
\midrule
\multicolumn{12}{l}{\textit{Open weights}} \\
\midrule

R1-Distill-Qwen-32B$^\dagger$ & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{62.1} & \textcolor{gray!135}{94.3} & \textcolor{gray!135}{90.0} & \textcolor{gray!135}{72.6} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{57.2} \\
s1-32B$^\dagger$ & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{57.6} & \textcolor{gray!135}{93.0} & \textcolor{gray!135}{-} & \textcolor{gray!135}{50.0} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} \\
% limo-32B$^\dagger$ & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{66.7} & \textcolor{gray!135}{94.8} & \textcolor{gray!135}{92.0} & \textcolor{gray!135}{57.1} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} & \textcolor{gray!135}{-} \\
Search-o1-32B$^\dagger$  & {77.9} & {\textbf{47.3}} & {\textbf{78.9}} & {\textbf{63.6}} & {86.4} & {85.0} & {56.7} & 57.7 & {32.4} & {20.4} & {33.0} \\
QwQ-32B-Preview & 75.6 & 39.8 & 68.4 & 58.1 & 90.6 & 80.0 & 50.0 &  &  & & 41.4 \\
\midrule
START (Ours) & \textbf{80.0} & \underline{46.2} & \underline{68.4} & \underline{63.6} & \textbf{94.4} & \textbf{95.0} & \underline{66.7} &  &  &  & \underline{46.4} \\
% \rowcolor[RGB]{236,244,252} 
% Search-o1-Light & \multicolumn{11}{l}{\textit{Results Coming Soon}} \\
\bottomrule
\end{tabular}
\end{table*}
